Object Placement Planning and Optimization for Robot Manipulators

We address the problem of motion planning for a robotic manipulator with the task to place a grasped object in a cluttered environment. In this task, we need to locate a collision-free pose for the object that a) facilitates the stable placement of the object, b) is reachable by the robot manipulator and c) optimizes a user-given placement objective. Because of the placement objective, this problem is more challenging than classical motion planning where the target pose is defined from the start. To solve this task, we propose an anytime algorithm that integrates sampling-based motion planning for the robot manipulator with a novel hierarchical search for suitable placement poses. We evaluate our approach on a dual-arm robot for two different placement objectives, and observe its effectiveness even in challenging scenarios.

==> sections/heuristics.tex <==
\section{Search Heuristics $\And$ Placement Predicate}
\subsection{Collision-cost}
\TODO{describe collision cost based on signed distance field and volumetric object representation}
\subsection{Dropping Heuristic}
\TODO{describe heuristic that takes falling length into account and uses placement planes
to estimate how suitable the surface is for placing}
\subsection{Physical Placement Model}
\TODO{describe physics model that we use to decide that we actually have a placement pose}



==> sections/method.tex <==
\section{Algorithm}
\TODO{First, outer loop algorithm that combines motion planner with goal sampler}
\subsection{Hierarchy Sampling}
\TODO{Explain that we utilize MCTS with FirstUrgency to sample regions from which
to start optimization. Explain rewards}
\subsection{Local search}
\TODO{Explain Jacobian descent}
\subsection{Motion Planner}
\TODO{Shortest: explain that we use BiRRT and update the trees every time a solution is found.
Might not require own section}

